CodeMatcher: Searching Code Based on Sequential Semantics of Important Query Words

To accelerate software development, developers frequently search and reuse existing code snippets from a large-scale codebase, e.g., GitHub. Over the years, researchers proposed many information retrieval based models for code search, but they fail to connect the semantic gap between query and code. An early successful deep learning based model DeepCS solved this issue by learning the relationship between pairs of code methods and corresponding natural language descriptions. Two major advantages of DeepCS are the capability of understanding irrelevant/noisy keywords and capturing sequential relationships between words in query and code. In this paper, we proposed an IR-based model CodeMatcher that inherits the advantages of DeepCS, while it can leverage the indexing technique in the IR-based model to accelerate the search response time substantially. CodeMatcher first collects metadata for query words to identify irrelevant/noisy ones, then iteratively performs fuzzy search with important query words on the codebase that is indexed by the Elasticsearch tool, and finally reranks a set of returned candidate code according to how the tokens in the candidate code snippet sequentially matched the important words in a query. We verified its effectiveness on a large-scale codebase with ~41k repositories. Experimental results showed that CodeMatcher achieves an MRR of 0.60, outperforming DeepCS, CodeHow, and UNIF by 82%, 62%, and 46% respectively. Our proposed model is over 1.2k times faster than DeepCS. Moreover, CodeMatcher outperforms GitHub and Google search by 46% and 33% respectively in terms of MRR. We also observed that: fusing the advantages of IR-based and DL-based models is promising; improving the quality of method naming helps code search, since method name plays an important role in connecting query and code.

==> road.tex <==
%!TEX root = main_tse.tex

Essentially, the code search aims to bridge the semantic gap between natural language and programming language, no matter for the deep-learning-based model DeepCS or the simplified model CodeMatcher. Therefore, this section analyzes the road ahead for code search under the view of linguistics between two languages with two related aspects: lexicon, and semantics via syntax.

\vspace{5pt}\noindent\textbf{Lexicon,} 
the used vocabulary. DeepCS fixed its vocabulary size to 10,000; thus, it will miss important new words from the frequently updated codebase and varied queries, and regarded new words as noises. It mitigates this issue by performing two steps: stemming words; addressing synonyms by the joint embedding technique. However, their capabilities are limited for large scale and dynamic codebase like GitHub. Also, we observed that the semantics of programming entity (e.g., File) in a query should be unique, but DeepCS may return code named with synonyms, leading to wrong search results.

To solve this problem, the proposed IR-based model CodeMatcher performed a fuzzy match between stemmed keywords in query and code. In this way, the whole indexed codebase can be regarded as vocabulary, and modifying codebase is equivalent to updating vocabulary. Besides, the fuzzy match can handle the compound issue. For example, the words "input stream" in query can match the compound word "inputstream" in the method. Meanwhile, CodeMatcher only generated synonyms for the verbs in queries that were not found in the codebase to control the usage of synonyms. But CodeMatcher also suffers from two lexical cases: \textit{(1) abbreviation,} simplifying 'initialize' to 'ini'; \textit{(2) acronym,} using the 'RMSD' to stand for the "root mean square deviation". Meanwhile, abbreviations and acronyms frequently occur in code. Thus it is worth incorporating code search models with more lexical features like abbreviation, acronym, and etc.

\SG{1}{Consider the importance of lexical factors in code search for the dynamic large-scale codebase, including new words, compound words, synonym, abbreviation, and acronym. Be careful to the uniqueness of class names from standard APIs in the query, which should not be replaced by synonyms.}

\vspace{5pt}\noindent\textbf{Semantics via syntax,} 
the meaning of a sentence is expressed by its structure. DeepCS leveraged RNN to embed query and code, assuming that their semantics are represented by the sequential relationship between words. However, we observed that for the query \textit{"convert int to string"} DeepCS returned many methods named by 'convertStringToInt'. In this case, DeepCS only learned the order of 'convert' and 'to' but missed the more important order of 'int', 'to', and 'string'.

To address this representation issue, CodeMatcher assigned higher weights on programming entities 'String' and 'Int', and reranked the returned methods whose name matched query keywords in order. Although this rule is straightforward and useful, it cannot capture high-level intent in query and code like DeepCS. Therefore, a better choice is to combine CodeMatcher with DeepCS. Moreover, both models cannot handle complex queries like "fastest way to determine if an integer's square root is an integer", so the syntactic structure of the query should be further considered carefully.

\SG{2}{Balance the pros and cons of CodeMatcher and DeepCS to build a better code search model, especially for the queries with complex syntax structure; pay more attention to the order of programming entities in a query.}

%\vspace{5pt}\noindent\textbf{Pragmatics,} 
%the way in which context contributes to meaning. DeepCS represented the semantics in code by a tuple of \textit{$\langle$method name, an API sequence, and token$\rangle$}, where APIs include constructor invocation and methods calls in the method body. This representation means that DeepCS divided the method body into API sequence and a set of tokens with bag-of-words assumption. However, DeepCS missed the semantic integrity of code in four aspects: \textit{(1) parameters,} it excluded the method parameters and returned type, which contributes much semantics for code; \textit{(2) programming entities,} the tokens in method body are just instances of programming types, which can be varied for different context; \textit{(3) token order,} the sequence of token in code should be meaningful, but the bag-of-words assumption missed this semantics and just treated it as common text; \textit{(4) divided context,} in the code, API sequence and tokens are sequentially mixed, so that the divided representation for method body could lose semantics in context. 

%To better maintain the semantic integrity and reduce the variation of customized context in code, CodeMatcher combined API sequence with token and represented as a sequence of fully qualified tokens, as described in Section \ref{method}. However, CodeMatcher still has two issues: \textit{(1) divided context,} it still divided a code context into method name and the other, and assign much higher weights on method name; \textit{(2) missed context,} it missed the code context in related comment and Javadoc, and Section \ref{github_search} highlights their importance for code search; \textit{(3) higher-level context,} Section \ref{optimum} shows that a code search maybe not method-level but class-level or even higher; \textit{(4) structural context,} it is lucky that CodeMatcher found the code for the query "breaking out of nested loops in java", but method name usually reflects its functional specification, not its structural information. Therefore, considering the structural context in code would be helpful for code search.

%\SG{3}{Consider the semantic integrity of a code context; pay more attention to higher-level context (e.g., class-level) and structural context for code search.}

To sum up, matching query tokens with method name and body strings as CodeMatcher is not enough for the code search task, especially for the queries with complex syntax structures. For the real-world code search, we only move one step further. For the road ahead, we suggest to combine the deep-learning-based model and the IR-based model and balance their pros and cons.

